Least-Squares Neural Network (LSNN) Method For Linear Advection-Reaction Equation: Non-constant Jumps

The least-squares ReLU neural network (LSNN) method was introduced and studied for solving linear advection-reaction equation with discontinuous solution in \cite{Cai2021linear,cai2023least}. The method is based on an equivalent least-squares formulation and \cite{cai2023least} employs ReLU neural network (NN) functions with $\lceil \log_2(d+1)\rceil+1$-layer representations for approximating solutions. In this paper, we show theoretically that the method is also capable of accurately approximating non-constant jumps along discontinuous interfaces that are not necessarily straight lines. Theoretical results are confirmed through multiple numerical examples with $d=2,3$ and various non-constant jumps and interface shapes, showing that the LSNN method with $\lceil \log_2(d+1)\rceil+1$ layers approximates solutions accurately with degrees of freedom less than that of mesh-based methods and without the common Gibbs phenomena along discontinuous interfaces having non-constant jumps.

==> nn_diagram.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}[]
\def\layersep{2.5cm}
\tikzset{%
  neuron missing/.style={
    draw=none, 
    scale=1.5,
    execute at begin node=$\vdots$
  },
}
\tikzstyle{neuron}=[circle,draw,minimum size=17pt]
\tikzstyle{input neuron}=[neuron, fill=green!50];
\tikzstyle{output neuron}=[neuron, fill=red!50];
\tikzstyle{hidden neuron}=[neuron, fill=blue!50];

\draw [dashed] (1/2*\layersep,0.9) -- (1/2*\layersep,-5.2);
\draw [dashed] (3*\layersep,0.9) -- (3*\layersep,-5.2);

\foreach \name / \y in {1,2,4}
\node[input neuron] (I-\name) at (0,-\y) {};
\node[neuron missing] (I-3) at (0,-2.9) {};


\foreach \name / \y in {1,2,3,5}
\path[yshift=0.5cm]
node[hidden neuron] (H1-\name) at (\layersep,-\y cm) {};
\path[yshift=0.5cm]
node[neuron missing] (H1-4) at (\layersep,-3.9cm) {};

\foreach \name / \y in {1,2,3,5}
\path[yshift=0.5cm]
node[hidden neuron] (H2-\name) at (3/2*\layersep,-\y cm) {};
\path[yshift=0.5cm]
node[neuron missing] (H2-4) at (3/2*\layersep,-3.9cm) {};
            
\foreach \name / \y in {1,2,3,5}
\path[yshift=0.5cm]
node[hidden neuron] (H3-\name) at (5/2*\layersep,-\y cm) {};
\path[yshift=0.5cm]
node[neuron missing] (H3-4) at (5/2*\layersep,-3.9cm) {};

% \path[yshift=0.5cm]
% node[output neuron] at (7/2*\layersep,-3cm) (O) {};

\foreach \name / \y in {1,2,4}
\node[output neuron] (O-\name) at (7/2*\layersep,-\y) {};
\node[neuron missing] (O-3) at (7/2*\layersep,-2.9) {};

\foreach \source in {1,2,4}
\foreach \dest in {1,2,3,5}
\path (I-\source) edge (H1-\dest);

\foreach \source in {1,2,3,5}
\foreach \dest in {1,2,3,5}
\path (H1-\source) edge (H2-\dest);

\foreach \source in {1,2,3,5}
\foreach \dest in {1,2,3,5}
\path (H2-\source) edge (H3-\dest);
            
\foreach \source in {1,2,3,5}
\foreach \dest in {1,2,4}
\path (H3-\source) edge (O-\dest);
    
\fill [white] (3/2*\layersep+1/4*\layersep,0cm) rectangle (3/2*\layersep+3/4*\layersep,-5cm);
        
\path[yshift=0.5cm]
node[scale=1.5] at (2*\layersep,-3cm) {$\cdots$};

\node[] at (0cm,0.7cm) {Input layer};
\node[] at (0cm,0.2cm) {$\mathbf{x}\in \mathbb{R}^d$};
\node[] at (\layersep+3/4*\layersep,0.7cm) {Hidden layers};
\node[] at (\layersep,0.2cm) {$N^{(1)}$};
\node[] at (3/2*\layersep,0.2cm) {$N^{(2)}$};
\node[] at (2*\layersep,0.2cm) {$\cdots$};
\node[] at (5/2*\layersep,0.2cm) {$N^{(L-1)}$};
\node[] at (7/2*\layersep,0.7cm) {Output layer};
\node[] at (7/2*\layersep,0.2cm) {$\mathcal{N}(\mathbf{x})\in \mathbb{R}^c$};

\end{tikzpicture}
\caption{ReLU Deep Neural Network}
\label{relu dnn figure}
\end{figure}
